Deep Reinforcement Learning for Online Optimal Execution Strategies

This paper tackles the challenge of learning non-Markovian optimal execution strategies in dynamic financial markets. We introduce a novel actor-critic algorithm based on Deep Deterministic Policy Gradient (DDPG) to address this issue, with a focus on transient price impact modeled by a general decay kernel. Through numerical experiments with various decay kernels, we show that our algorithm successfully approximates the optimal execution strategy. Additionally, the proposed algorithm demonstrates adaptability to evolving market conditions, where parameters fluctuate over time. Our findings also show that modern reinforcement learning algorithms can provide a solution that reduces the need for frequent and inefficient human intervention in optimal execution tasks.

==> tables_experiment.tex <==

\begin{table}[h!]
  \centering
  \begin{threeparttable}
  \resizebox{1\textwidth}{!}{%
  \begin{tabular}{l | l l l}
  \toprule
    \hline
  \textbf{Notation} & \textbf{Value} & \textbf{Description} & \textbf{Section} \\
  \hline
  \multicolumn{4}{l}{\textbf{Environment parameters}} \\
   \hline
    $T$ & $10, 25, 50$ & Time horizon& Section~\ref{sec:market_impact_model} \\
   $P_{0}^{0}$ & $50$ & Initial price & Section~\ref{sec:market_impact_model} \\
   $X_{0}$ & $10$ & Initial inventory & Section~\ref{sec:market_impact_model} \\
   $\kappa$ & $1$ & Scale parameter of exponential kernel & Section~\ref{sec:market_impact_model} \\
   $\rho$ & $[0.5, 1]$ & Decay parameter of exponential kernel & Section~\ref{sec:market_impact_model} \\
   $\sigma_{W}$ & $0.0001$ & Variance of the unaffected price process & Section~\ref{sec:experiment_set_up} \\[0.2cm]
   \hline 
    \multicolumn{4}{l}{\textbf{DDPG parameters}} \\
    \hline
  $L^{\text{critic}}$ & XX & Number of hidden layer of critic network & Section~\ref{sec-deep-dpg} \\
  $n_h^{\text{critic}}$ & XX & Number of hidden units of critic network & Section~\ref{sec-deep-dpg} \\
  $L^{\text{actor}}$ & XX & Number of hidden layer of actor network & Section~\ref{sec-deep-dpg} \\
  $n_h^{\text{actor}}$ & XX & Number of hidden units of actor network & Section~\ref{sec-deep-dpg} \\
  $\tau_{\phi}$ & XX & Update rate from policy to target critic network & Section~\ref{sec-deep-dpg} \\
  $\tau_{\theta}$ & XX & Update rate from policy to target actor network & Section~\ref{sec-deep-dpg} \\
  $D$ & XX & Buffer size & Section~\ref{sec-deep-dpg} \\
  $B$ & XX & Batch size & Section~\ref{sec-deep-dpg} \\
  $\ell^{\text{critic}}$ & XX & Learning rate of critic network's optimizer & Section~\ref{sec-deep-dpg} \\
  $\ell^{\text{actor}}$ & XX & Learning rate of actor network's optimizer & Section~\ref{sec-deep-dpg} \\
  $\theta_{\varepsilon}$, $\sigma_{\varepsilon}$ & XX &  Parameters of Ornstein-Uhlenbeck noise process & Section~\ref{sec-deep-dpg} \\
  $\varepsilon$ & XX & Probability of exploring at the start of the experiment & Section~\ref{sec-deep-dpg} \\
  $\varepsilon^{\text{decay}}$ & XX & Decay on the probability of exploring  & Section~\ref{sec-deep-dpg} \\
$\varepsilon^{\text{min}}$ & XX & Minimum probability of exploring at any time & Section~\ref{sec-deep-dpg} \\
\hline
    \bottomrule
  \end{tabular}}
  \end{threeparttable}
    \caption{\textbf{Parameters of environment and DDPG used in the numerical experiments.} } 
    
  \label{tab:convergence_experiment_parameters}
\end{table}
